Stochastic Ray Tracing for the Reconstruction of 3D Gaussian Splatting

Ray-tracing-based 3D Gaussian splatting (3DGS) methods overcome the limitations of rasterization -- rigid pinhole camera assumptions, inaccurate shadows, and lack of native reflection or refraction -- but remain slower due to the cost of sorting all intersecting Gaussians along every ray. Moreover, existing ray-tracing methods still rely on rasterization-style approximations such as shadow mapping for relightable scenes, undermining the generality that ray tracing promises. We present a differentiable, sorting-free stochastic formulation for ray-traced 3DGS -- the first framework that uses stochastic ray tracing to both reconstruct and render standard and relightable 3DGS scenes. At its core is an unbiased Monte Carlo estimator for pixel-color gradients that evaluates only a small sampled subset of Gaussians per ray, bypassing the need for sorting. For standard 3DGS, our method matches the reconstruction quality and speed of rasterization-based 3DGS while substantially outperforming sorting-based ray tracing. For relightable 3DGS, the same stochastic estimator drives per-Gaussian shading with fully ray-traced shadow rays, delivering notably higher reconstruction fidelity than prior work.

==> sec/relight_figure.tex <==

\begin{figure}[]
    \setlength{\resLen}{0.8in}
    %
    \centering
    \small
    \addtolength{\tabcolsep}{-5.5pt}
    %
    %
    \begin{tabular}{cccc}
        % &
        (a) \textbf{Ref} & (b) \textbf{Ours} & (c) \textbf{Relit1} & (d) \textbf{Relit2}
        \\ \vspace{-0.1em}
        \includegraphics[trim={0pt 110pt 0pt 0pt},clip,width=\resLen]{images/relightable/cat/ref_orig.jpg} &
        \includegraphics[trim={0pt 110pt 0pt 0pt},clip,width=\resLen]{images/relightable/cat/ours_orig.jpg} &
        \includegraphics[trim={0pt 110pt 0pt 0pt},clip,width=\resLen]{images/relightable/cat/ours_relit1_.jpg} &
        \includegraphics[trim={0pt 110pt 0pt 0pt},clip,width=\resLen]{images/relightable/cat/ours_relit2.jpg}
    \end{tabular}
    %
    \caption{
        Visualization of reconstruction and relighting for the \textit{Cat} scene. We show the reference (a), our reconstruction (b), and relighting under two novel lighting setups (c-d) not present in the training data.
    }
    \label{fig:rebuttal_relight}
\end{figure}

==> sec/tab_benchmark_ssplats.tex <==
\begin{table*}[t]
    \caption{\label{tab:benchmarks}
        \textbf{Novel view synthesis}: Results for our approach and baselines on a variety of novel view synthesis benchmarks. As a \textbf{ray tracing} algorithm, our method runs at similar speed to the rasterization-based baseline, and achieves comparable performance on all benchmarks.
    }
    \centering
    \small
    \begin{threeparttable}
        \footnotesize % or \footnotesize for slightly larger text
        \setlength{\tabcolsep}{4.2pt} % reduce horizontal padding between columns
        \begin{tabular}{
            l
            S[table-format=2.2] S[table-format=1.3] S[table-format=1.3] l
            S[table-format=2.2] S[table-format=1.3] S[table-format=1.3] l
            S[table-format=2.2] S[table-format=1.3] S[table-format=1.3] l
        }
        \toprule
        \multirow{2}{*}{Method\textbackslash Metric}
         & \multicolumn{4}{c}{\textbf{MipNeRF360}} 
         & \multicolumn{4}{c}{\textbf{Tanks \& Temples}}
         & \multicolumn{4}{c}{\textbf{Deep Blending}} \\
        \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
         & {PSNR$\uparrow$} & {SSIM$\uparrow$} & {LPIPS$\downarrow$} & {Time$\downarrow$}
         & {PSNR$\uparrow$} & {SSIM$\uparrow$} & {LPIPS$\downarrow$} & {Time$\downarrow$}
         & {PSNR$\uparrow$} & {SSIM$\uparrow$} & {LPIPS$\downarrow$} & {Time$\downarrow$} \\
        \midrule
        3DGS           & 28.69 & 0.867 & 0.224 & 24m & 23.14 & 0.853 & \text{-} & 14m & 29.41 & 0.903 & \text{-} & 20m \\
        3DGRT          & 28.40 & 0.862 & 0.233 & 69m & 22.95 & 0.838 & 0.221 & 41m & 29.69 & 0.904 & 0.318 & 54m \\
        %Ours           & 28.05 & 0.852 & 0.251   & {} & {} & {} & {} & {} & {} & {} & {} \\
        \textbf{Ours} (15spp)     & 27.90 & 0.843 & 0.265 & 37m & 22.37 & 0.821 & 0.233 & 21m & 29.51 & 0.902 & 0.330 & 24m \\
        \textbf{Ours} (30spp)     & 28.14 & 0.850 & 0.254 & 52m & 22.75 & 0.827 & 0.229 & 25m & 29.75 & 0.904 & 0.327 & 29m \\
        %Stoch-Splats   & 24.67 & 0.714 & 0.392 & {1h23m23s} & {} & {} & {} & {} & {} & {} & {} & {} \\
        \bottomrule
        \end{tabular}
    \end{threeparttable}
\end{table*}

